Dr-COVID: Graph Neural Networks for SARS-CoV-2 Drug Repurposing

The 2019 novel coronavirus (SARS-CoV-2) pandemic has resulted in more than a million deaths, high morbidities, and economic distress worldwide. There is an urgent need to identify medications that would treat and prevent novel diseases like the 2019 coronavirus disease (COVID-19). Drug repurposing is a promising strategy to discover new medical indications of the existing approved drugs due to several advantages in terms of the costs, safety factors, and quick results compared to new drug design and discovery. In this work, we explore computational data-driven methods for drug repurposing and propose a dedicated graph neural network (GNN) based drug repurposing model, called Dr-COVID. Although we analyze the predicted drugs in detail for COVID-19, the model is generic and can be used for any novel diseases. We construct a four-layered heterogeneous graph to model the complex interactions between drugs, diseases, genes, and anatomies. We pose drug repurposing as a link prediction problem. Specifically, we design an encoder based on the scalable inceptive graph neural network (SIGN) to generate embeddings for all the nodes in the four-layered graph and propose a quadratic norm scorer as a decoder to predict treatment for a disease. We provide a detailed analysis of the 150 potential drugs (such as Dexamethasone, Ivermectin) predicted by Dr-COVID for COVID-19 from different pharmacological classes (e.g., corticosteroids, antivirals, antiparasitic). Out of these 150 drugs, 46 drugs are currently in clinical trials. Dr-COVID is evaluated in terms of its prediction performance and its ability to rank the known treatment drugs for diseases as high as possible. For a majority of the diseases, Dr-COVID ranks the actual treatment drug in the top 15.

==> sections/Experiments.tex <==
\section{Experimental Setup}  \label{sec:Exp}
In this subsection, we evaluate our model performance and discuss on the choice of hyper-parameters. We see this link prediction task as a binary classification problem where a positive class represents the existence of a link between the input drug and disease and otherwise for a negative class. We have 6113 positive samples (true drug-disease links) in our dataset. To account for the negative class samples, we randomly choose 200,000 false drug-disease pairs (i.e., there is no link between drugs and diseases). These links are then divided into the training and testing set with a $90\%-10\%$ split. To use mini batch stochastic gradient descent, we group our training set in batches of size 512 and train them for 20 epochs. Due to the significant class imbalance, we oversample the true drug-disease links while creating batches, and thus maintaining the class ratio (number of negative samples to positive samples) of $1.5$ in each batch. Typically, the weight $w$ on the positives samples (mentioned in \eqref{eq:Loss}), is also chosen to be the class imbalance ratio of each batch. Hence, we fix $w$ to be $1.5$.


We perform experiments on three sequential GNN architectures, namely, GCN~\cite{GCN}, GraphSAGE~\cite{GraphSAGE} and GAT~\cite{GAT} for the ldrug repurposing task, which we treat as a link prediction problem, and compare with our proposed \texttt{Dr-CoV} architecture. Specifically, the SIGN encoder in  \texttt{Dr-CoV} is replaced with GCN, GraphSAGE and GAT to evaluate the model performance. Two blocks of these sequential models are stacked to maintain the consistency with $r=2$ of our architecture. We evaluate these models on the testing links, which are known treatments for diseases that are not shown to the model while training. The model is evaluated based on two performance measures. Firstly, we report the ability to classify the links correctly, i.e., to predict the known treatments correctly for diseases in test set. This is measured through the area under the probability curves, known as receiver operating characteristic (ROC) curves of the true positive rate (TPR) versus the false positive rates (FPR). Next, using a list of predicted drugs for the diseases in the test set, we report that model's ability to rank (obtained by ordering the scores in \eqref{eq:Scorer}) the actual treatment drug as high as possible. 
\\
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{Images/ROC_curves.png}
    \caption{ROC Curves}
    \label{fig:ROC}
\end{figure}
ROC curves show the performance of a binary classification model, by varying the threshold values used to classify the positive samples, which eventually changes the TPR and FPR. We can infer about the separation ability of a classifier by computing the area under ROC (AUROC) which lies in [0,1], wherein 1 indicates the best performance, 0.5 tells that the model is unable to discriminate between the classes (random classifier) and 0 indicates a completely opposite behaviour. Figure \ref{fig:ROC} shows the ROC curves of different GNN models. We can see that all the models have very similar AUROC values. 


Secondly, we compare in terms of the rank of the actual treatment drug in the predicted list for a disease from the testing set, where the rank is computed by ordering the scores. Additionally, we also report the network proximity scores~\cite{DR_M_1}, rank drugs based on these scores and compare with other encoder models. These network proximity scores are a measure of the shortest distance between drug and disease target genes. They are computed as: 

\[d_{CT} = \frac{1}{||C||+||T||}(\sum_{c\in C}min_{t\in T}d(c,t) + \sum_{t \in T}min_{c\in C}d(c,t)) \label{eq:dct} \tag{\ding{6}}\
\]
where $\cal{C}$ is a set of drug target genes, $\cal{T}$ of disease target genes and $d(c_i,t_j)$ is the shortest distance between gene $c_i \in \cal{C}$ and gene $t_j \in \cal{T}$ in the gene interactome. We convert these into Z-scores using the permutation tests as 
\[Z_{d_{CT}} = \frac{d_{CT}-\bar{d}_r}{\sigma_r} \label{eq:Z_score} \tag{\ding{7}}\
\]
where we randomly select gene lists with the same degree distributions that of $\cal{C}$ and $\cal{T}$ and compute the mean score $\bar{d}_r$ and its standard deviation $\sigma_r$. Table 1 gives this ranking performance comparison, which clearly shows that the SIGN architecture has a better ranks on the unseen diseases than the other GNN variants. It is also evident that the diseases on which we evaluate are not confined to a single anatomy (e.g., \emph{rectal neoplasms} are majorly confined to the \emph{rectum} anatomy, whereas \emph{pulmonary fibrosis} is a \emph{lung} disease), nor do they require a similar family of drugs for their treatment (e.g., \emph{Fluorouracil} is an antineoplastic drug and \emoh{Prednisone} is an anti-inflammatory corticosteroid) showcasing our model's unbiased nature. We give more importance to the ranking parameter as any drug predictor would require to classify and then rank the correct drugs as high as possible. Considering this AUROC-ranking trade-off we can see that \textttt{Dr-CoV} with SIGN encoder performs the best. Our complete implementation is available at \href{https://github.com/siddhant-doshi/Drug_repurposing}{\textit{https://github.com/siddhant-doshi/Drug\_repurposing}}

\\
\begin{table*}[!htbp]
    \centering
    \begin{tabular}{*7c}
        \hline
        \hline
        Disease &  Treatment drug & \multicolumn{5}{c}{Ranks}\\
        {}   & {}   & SIGN   & SAGE & GCN & GAT & Network proximity\\
        \hline
        Encephalitis & Acyclovir & 10 & 35 & 35 & 295 & 5462\\
        Rectal neoplasms & Fluorouracil & 9 & 421 & 16 & 231 & 2831\\
        Pulmonary fibrosis & Prednisone & 5 & 3 & 10 & 9 & 2072\\
        Atrioventricular block & Atropine & 6 & 79 & 8 & 14 & 4453\\
        Pellagra & Niacin & 2 & 56 & 497 & 484 & Not computable\textsuperscript{4} \\
        Colic & Hyoscyamine & 1 & 1 & 501 & 205 & Not computable\textsuperscript{4} \\ 
        Leukemia & Azacitidine & 17 & 120 & 31 & 332 & 377 \\
        \hline
        \hline
    \end{tabular}
    \caption{Ranking table}
\end{table*}
\\
%\tablefootnote{\label{xx}There are no associated genes with the disease in our database, which makes it impossible to compute the Z scores.}%
%\textsuperscript{a}
\footnotetext{There are no associated genes with the disease in our database, which makes it impossible to compute the Z scores.}
\textbf{COVID analysis - } We perform a similar analysis and identify potential candidate drugs for SARS-CoV-2. For all the COVID related nodes in our dataset comprising 27 proteins, SARS virus, IBV, MERS, CoV-229E, CoV-NL63 and MHV we individually predict the drugs for all these 33 nodes. Each protein in SARS-CoV-2 targets a different set of genes in humans, so we think it is effective to have individual predictions. We then pick the top 10 drugs from all the predicted drug sets and give out a list of 150 possible candidates that we think might be promising in fighting against COVID, of which 35 are currently in clinical trials. Our predictions have a mixture of antivirals, antineoplastic, corticosteroids, monoclonal antibodies (mAb), non-steroidal anti-inflammatory drugs (NSAIDs), angiotensin-converting enzyme (ACE) inhibitors, statin family of drugs and some of the vaccines discovered previously for other diseases. We discuss the COVID analysis in a more detailed manner in the Results section.

==> sections/Overview_GNN.tex <==
\section{Overview of Graph neural networks} \label{sec:GNN}
Geometric Deep Learning (GDL)~\cite{Bronstein} referred to as deep learning on graphs, has recently emerged as one of the exciting topics in deep learning. They deal with non-structured and more realistic data, beyond the Euclidean space that can be represented in the form of graphs. GNN tend to generalize the traditional convolution operation of the convolutional neural network (CNN) on such graph-structured data. Some of the properties possessed by CNNs like local connectivity - nearby pixels being highly correlated, shift invariance - model learns despite the spatial positions of pixels, and generalizing over any input dimension serves an attractive base for analyzing the non-structured data. GNNs also draw their core from these and possess some similar properties like connected nodes are supposed to be highly correlated, the capability to process position invariant data and analyze any sized input graph. The main idea is to generate low-dimensional embeddings for nodes in a graph by considering the complete graph connectivity, so that these embeddings can further assist in many tasks like node classification, link prediction, etc. Broadly convolutions over graphs are categorized into two sections - spectral and spatial.
\\
\\
\textbf{Spectral} based approaches have their roots in spectral theory and graph signal processing~\cite{Frossard}~\cite{Moura}~\cite{Sandryhaila}. Any undirected graph $G$ is represented using it's normalized laplacian $\textbf{L} = \textbf{I}-\textbf{D}^{-\frac{1}{2}}\textbf{AD}^{-\frac{1}{2}}$, where $\textbf{D}$ is a diagonal degree matrix and $\textbf{A}$ is the adjacency matrix of $G$. The well known convolution theorem - spatial convolution equals multiplication in frequency domain, can also be applied over graphs by just replacing the basis DFT matrix with the eigen vectors of the normalized laplacian $\textbf{L}$. A graph signal $\textbf{x}\in \textbf{R}^\textbf{n}$ over a graph $G$ is a signal that represents the information about the nodes i.e $x_i$ would represent the information about the $i^{th}$ node. The graph convolution operation of a signal $\textbf{x}$ over $G$ with some graph filter $\textbf{g}\in \textbf{R}^\textbf{n}$ is defined as - 
\[\textbf{x} *_G \textbf{g} = \textbf{U}(\textbf{U}^\textbf{T}\textbf{x} \odot \textbf{U}^\textbf{T}\textbf{g}) \label{eq:Conv_1} \tag{\ding{1}}\]
$\textbf{U}^\textbf{T}\textbf{x}$ and $\textbf{Ux}$ represent fourier and inverse fourier transform of a graph signal $\textbf{x}\in \textbf{R}^\textbf{n}$ over $G$, where $\textbf{U}$ is eigen vector matrix of $\textbf{L}$ and $\odot$ represents the hadamard product. We can further simplify \eqref{eq:Conv_1} by choosing a filter $\textbf{g}_\theta = diag(\textbf{U}^\textbf{T}\textbf{x})$ to - 
\[\textbf{x} *_G \textbf{g}_\theta = \textbf{Ug}_\theta \textbf{U}^\textbf{T}\textbf{x} \label{eq:Conv_2} \tag{\ding{2}} \]
All the spectral based convolutional GNNs revolve around this \eqref{eq:Conv_2} with different choice of filters $\textbf{g}_\theta$. Major limitation of such spectral based methods is the high computational cost, $O(n^3)$ of the eigen decomposition of $\textbf{L}$. ChebNet\cite{ChebNet} and GCN\cite{GCN} help in reducing this cost by approximating the filter $\textbf{g}_\theta$ with chebyshev polynomial of the eigen value matrix. \\
\\ \textbf{Graph convolutional network (GCN)} serve as a bridge between the spectral and the spatial methods. They simplified these spectral models by approximating the filter $\textbf{g}_\theta$ using first order chebyshev polynomials.
\[\textbf{H} = \textbf{X} *_G \textbf{g}_\Theta = f(\tilde{\textbf{A}}\textbf{X}\Theta) \label{eq:GCN} \tag{\ding{3}} \]
where $f(\cdot)$ is a non-linear activation function, $\tilde{\textbf{A}} = \textbf{I} +  \textbf{D}^{-\frac{1}{2}}\textbf{A}\textbf{D}^{-\frac{1}{2}}$ is the normalized adjacency matrix of $G$ with $\textbf{I}$ to account for the self embeddings, $\textbf{H}$ is the new representation of the nodes, which we generally refer to as the embedding matrix and $\textbf{X}$ is a matrix of all the graph signals stacked together. The relaxation on $\textbf{g}_\theta$ provided by GCN popularized the spatial methods.
\\
\\
\textbf{Spatial} based approaches are analogous to the CNNs in a way where we capture the similarity between two connected nodes in a graph. Images can be considered as a particular case of Euclidean or an ordered graph where nearby pixels are connected. We process these images by moving a spatial filter over them and getting new representations of the pixels, which are nothing but transformed information from its nearby pixels (neighbours). Using this same analogy in graph convolutions we get a new representation for a node by combining information from its neighbour nodes. We can gather information from its K-hop neighbours by stacking such K message passing blocks, similar to how we stack these CNN blocks. The node embeddings can be represented as -  
\[\ \textbf{h}_v^{(k+1)} = f(\textbf{h}_v^{(k)} + \sum_{j\in N(v)}\textbf{W}^{(k)}\textbf{h}_j^{(k)}) \label{eq:GCN1} \tag{\ding{4}} \]
$\textbf{h}_v^{(k)}$ represent the $k^{th}$ layer embedding for a node $v$ and $\textbf{W}^{(k)}$ is a learnable transformation matrix in the $k^{th}$ layer. The neural network for graphs (NN4G)~\cite{NN4G} was the first work proposed. Eventually many algorithms like DCNN~\cite{DCNN}, MPNN~\cite{MPNN}, GIN~\cite{GIN}, GraphSAGE~\cite{GraphSAGE}, GAT~\cite{GAT}, SIGN~\cite{SIGN} came up in this direction. DCNN considered this message passing as a diffusion process, meaning nodes transfer information with some transition probability to achieve equilibrium after some rounds. MPNN outlined a general framework for message passing and tried to club the existing methods into that framework. Shortcomings in MPNN were identified and solved by GIN. GAT gave individual attention to neighbour nodes instead of treating everyone equally. To address the issue of scalability, GraphSAGE proposed a neighbour sampling method i.e. instead of taking the entire neighbourhood, we can randomly sample a subset of neighbour nodes. SIGN model takes a different approach to solve the scalability issue and introduce a flavour of parallelism. We will describe the SIGN architecture in detail in the Methods section with respect to our drug repurposing model.   
\\
\\
Spatial models have the upper hand compared to the spectral models in - i) Efficiency ii) They are inductive models meaning they are not restricted with the graph size they train on. They tend to perform better on the unseen data than the spectral models iii) Easily scalable to large graphs iv) Their performance is insensitive to small perturbations to the graph compared to that of the spectral models. 

==> sections/author_summary.tex <==
\section*{Author summary} \label{sec:auth_summary}
The availability of large volumes of biological data has enhanced the understanding of various biological systems. Data-driven computational techniques in fields like biology, medicine, genomics, and neuroscience are gaining attention due to advances in artificial intelligence and machine learning tools. We apply recent tools from artificial intelligence to drug repurposing for the 2019 novel coronavirus diseases (COVID-19). Specifically, we propose a graph neural network (GNN) model to capture local and structural information in a complex interaction network comprising drugs, diseases, genes, and anatomies as entities. The proposed graph neural network model learns from known treatments of many diseases and complex interactions between the four entities and successfully predicts unknown links between approved drugs and novel diseases, such as COVID-19.

==> sections/final.tex <==
\section*{Abstract}
The \emph{2019 novel coronavirus (SARS-CoV-2)} pandemic has resulted in more than a million deaths, high morbidities, and economic distress worldwide. There is an urgent need to identify medications that would treat and prevent novel diseases like the 2019 coronavirus disease (COVID-19). Drug repurposing is a promising strategy to discover new medical indications of the existing approved drugs due to several advantages in terms of the costs, safety factors, and quick results compared to new drug design and discovery. In this work, we explore computational data-driven methods for drug repurposing and propose a dedicated graph neural network (GNN) based drug repurposing model, called \texttt{Dr-COVID}. Although we analyze the predicted drugs in detail for COVID-19, the model is generic and can be used for any novel diseases. We construct a four-layered heterogeneous graph to model the complex interactions between drugs, diseases, genes, and anatomies. We pose drug repurposing as a link prediction problem. Specifically, we design an encoder based on the scalable inceptive graph neural network (\texttt{SIGN}) to generate embeddings for all the nodes in the four-layered graph and propose a quadratic norm scorer as a decoder to predict a treatment possible for a disease. We provide a detailed analysis of the 150 potential drugs (such as \emph{Dexamethasone}, \emph{Ivermectin}) predicted by \texttt{Dr-COVID} for COVID-19 from different pharmacological classes (e.g., corticosteroids, antivirals, antiparasitic). Out of these 150 drugs, 46 drugs are currently in clinical trials. \texttt{Dr-COVID}  is evaluated in terms of its prediction performance and its ability to rank the known treatment drugs for diseases as high as possible. For a majority of the diseases, \texttt{Dr-COVID} ranks the actual treatment drug in the top 15.

==> sections/ref.tex <==
\section*{References} \label{sec:references}

\printbibliography[heading=none]
